Cup Products and Pairings for Abelian Varieties

Let $A_K$ be an abelian variety with semistable reduction over a strictly henselian field of positive characteristic with perfect residue class field. We show that there is a close connection between the pairings of Grothendieck, Bester/Bertapelle and Shafarevic. In particular, we show that the pairing of Bester/Bertapelle can be used to describe the $p$-part of Grothendieck's pairing in the semistable reduction case, thus proving a conjecture of Bertapelle.

==> cup.tex <==
\chapter{The Cup Product for Strictly Henselian Fields}


\section{The Galois Group of a Strictly Henselian Field}\label{gal_ksh}

In this section, we recall the structure of the Galois group of a discretely valuated, strictly
henselian field $K$. The structure has important consequences for the properties of the cohomology
of $K$ and for the reduction behaviour of abelian varieties over $K$. We are going to study the
latter aspect in the third chapter.
\par
The key to the first proposition is the theory of \emph{tamely ramified extensions}: Let $R$ be a
henselian, discrete valuation ring with field of fractions $K=\quot R$ and residue class field $k$
of characteristic $p\neq 0$. Let $L/K$ be a finite Galois extension of $K$. Since $R$ is henselian,
the integral closure $S$ of $R$ in $L$ is a henselian, discrete valuation ring with residue class
field $\ell$. Remember that such an extension $L/K$ is said to be \emph{tamely ramified} if its
residue class field extension $\ell/k$ is separable and if its ramification index $e_{L/K}$ is prime
to the characteristic $p$ of the residue class field.\index{tamely ramified
extension} 
\par
In the following, we will work over a strictly henselian, discrete valuation ring $R$:

\begin{prop}\label{gal_k}
Let $R$ be a strictly henselian discrete valuation ring with field of fractions $K$ and residue
class field $k$ of characteristic $p\neq 0$.
\begin{enumprop}
  \item A finite extension $L/K$ is tamely ramified if and only if $p\nmid[L:K]$. Each such
   extension   is a cyclic Galois extension.
  \item Let $L/K$ be any finite Galois extension with Galois group $G=\gal(L/K)$. Then there 
  exists a unique $p$-Sylow-subgroup $G_p\sub G$.
\end{enumprop}\index{wildly ramified extension}\index{tamely ramified extension}
Consequently, any Galois extension $L/K$ with Galois group $G$ can be splitted up into a tamely
ramified
Galois extensions $L^\tr/K$ with cyclic Galois group and a wildly ramified Galois extension
$L/L^\tr$ with Galois group $G_p$, where $G_p\sub G$ is the unique $p$-Sylow-subgroup
of $G$.
\end{prop}


\begin{proof}
Since $k$ is separably closed, every finite extension  $\ell/k$ is purely inseparable and, hence,
its degree is a power of  $p$. Due to the fundamental equation $[L:K]=e_{L/K}\cdot[\ell/k]$ the
first part of \enum 1 is obvious.
\par
Since $R$ is henselian, we can lift the roots of the polynomial $X^n-1$ from $k$ to $R$. Thus, we
can conclude that the $n$-th roots of unity are contained in $R$ and hence in $K$. Any extension
$L/K$ of degree $n$ prime to $p$ can easily be shown to be a Kummer extension\index{Kummer
extension}, isomorphic to
\[
L\iso K[X]\mod (X^n-\pi)
\]
for a suitable uniformising element $\pi$ of $K$. Now,
\[
\sigma\longmapsto \frac {\sigma(X)} X
\]
constitutes an isomorphism $\gal(L/K)\isoto\mu_n(K)$.  Since the $n$-th roots of unity are
contained in $R$ and thus in $K$, the group $\mu_n(K)$ is (non canonically) isomorphic to $\bbZ\mod
n$. This settles assertion \enum 1. To show \enum 2, let $G_p$ be any $p$-Sylow subgroup of $G$. The
degree of the corresponding field extension $L^{G_p}/K$ is prime to $p$. Hence it is a Galois
extension by \enum 1, which implies that $G_p$ is normal. 
\end{proof}

We write $K_s^\tr$ for the union of all tamely ramified extensions of $K$ in a fixed separable
closure $K_s$ of $K$. The field $K_s^\tr$ is tamely ramified over $K$, and the above proposition can
be generalised to the situation of profinite Galois groups.\index{profinite group} Recall that for a
prime $\ell$ the ring of $\ell$-adic numbers is defined to be
\[
\hat\bbZ_\ell\defeq\projlim_{n\in\bbN}\bbZ\mod \ell^n.
\]
Moreover, we will need the ring $\hat\bbZ\defeq\prod_{\ell}\hat\bbZ_\ell$. 

\begin{cor}\label{galK_seq}
Let $K$ be the quotient field of a strictly henselian discrete valuation ring. There exists an
exact sequence
\[
0\longto P\longto\gal(K_s/K)\longto\prod_{\ell\neq p}\hat\bbZ_\ell\longto 0
\]
with the pro-$p$-group $P=\gal(K_s/K_s^\tr)$. The last term is isomorphic to the Galois group
$\gal(K_s^\tr/K)$. \qed
\end{cor}


Let us recall that a profinite group $P$ is called a \emph{pro-$p$-group}\index{pro-$p$-group},
if $P\mod P'$ is a $p$-group for every open subgroup $P'\sub P$.
\par
Let $L/K$ be a finite Galois extension and let  $G'\defeq\gal(K_s/L)$ be the absolute Galois group
of $L$. Due to proposition
\ref{gal_k} it gives rise to Galois extensions $K\sub L^\tr\sub L$.  For later use, we want 
to examine the wildly ramified extension $K_s/L^\tr$ and its Galois group.


\begin{prop}\label{gal_Ltr}
In this situation, the field $L^\tr$ can be written as $L\cap K_s^\tr$. Thus, we have
$\gal(K_s/L^\tr)=G'\cdot P$ for the pro-$p$-group $P=\gal(K_s/K_s^\tr)$.
\end{prop}



\begin{proof}
Since $K_s^\tr$ is the union of all tamely ramified extensions of $K$ in $K_s$, it is a tamely
ramified extension of $K$. Thus, $K_s^\tr\cap L$ is the maximal tamely ramified extension of $K$ in
$L$.
\end{proof}



\section{Duality for Galois Cohomology}

This section is due to \cite{sga5}, I, 5.1.8. Still, we take $R$ to be a strictly henselian
discrete valuation ring with quotient field $K$ and residue class field $k$ of characteristic
$p\neq 0$. Let $n$ be an integer with $(n,p)=1$. It is clear by Hensel's Lemma that $\mu_{n,K}$
is (non-canonically) isomorphic to the constant group scheme $\bbZ\mod n$ and that the map $x\mapsto
x^n$ on $R^\ast$ is surjective. Using this fact, our first cohomological observation is the
following lemma:

\begin{lemma}\label{hensel_coh}
Let $n$ be prime to $p$. We have $\HH^1(K,\mu_{n,K})=\bbZ\mod n$.
\end{lemma}


\begin{proof}
The Kummer sequence\index{Kummer sequence}
\[
0\longto\mu_{n,K}\longto\bbG_{m,K}\Longto n\bbG_{m,K}\longto 0
\]
induces the following part of the long exact cohomology sequence:
\[
K^\ast\Longto n K^\ast\longto\HH^1(K,\mu_{n,K})\longto\HH^1(K,\bbG_{m,K}).
\]
The last group is trivial due to Hilbert 90. Thus, $\HH^1(K,\mu_{n,K})$ is canonically isomorphic to
$K^\ast\mod
(K^\ast)^n$. Applying the snake lemma to the diagram with exact rows
\begin{diagram}
0 & \rTo & R^\ast & \rTo & K^\ast & \rTo^\nu & \bbZ & \rTo & 0 \\
  &      & \dTo>n &      & \dTo>n &          & \dTo>n \\
0 & \rTo & R^\ast & \rTo & K^\ast & \rTo^\nu & \bbZ & \rTo & 0
\end{diagram}
leads to the assertion.
\end{proof}


Let us recall that the  categories of finite, \'etale $K$-group schemes and the category of finite,
continuous $G$-modules for $G\defeq \gal(K_s/K)$ are equivalent. This equivalence is induced by
$N\mapsto N(K_s)$.  In particular, we can use Galois cohomology\index{Galois cohomology|see{group
cohomology}}\index{group cohomology} to compute the cohomology of finite,
\'etale group schemes over $K$. \label{group_coh_cup}It is known that group cohomology is equipped
with a functorial cup product, \cite{Br}, V.3.\index{cup product!of group cohomology} Let us give a
brief introduction to cup products. Later, in chapter \ref{cup_derived} we will treat
cup products in greater generality. The cup product of group cohomology is a
family of functorial morphisms
\[
\HH^r(G,M)\times\HH^s(G,N)\longto\HH^{r+s}(G,M\tensor N),
\]
for continuous $G$-modules $M$ and $N$ and every pair of integers $r,s\geq 0$. For $r=s=0$ the cup
product coincides with the canonical pairing $M^G\times N^G\to (M\tensor N)^G$.  For now, let us
remark that the cup product is  induced by the following product defined on the
Bar-resolution\index{Bar-resolution} of $M$ and $N$ and $M\tensor N$ by the \emph{Alexander-Whitney
formula}\index{Alexander-Whitney formula}
\begin{equation}\label{grp_coh_alex_whit}
 (m\cup n)(g_1,\ldots,g_{r+s})\defeq (-1)^{r+s}m(g_1,\ldots,g_r)\tensor g_1\cdot\ldots\cdot
g_r\cdot n(g_{r+1},\ldots,g_{r+s}) 
\end{equation}
for cochains $m\colon G^r\to M$ and $n\colon G^s\to N$.
\par
We are interested in the case of a finite, \'etale $K$-group scheme $N$ whose order $n$ is prime to
$p$. Its \emph{Cartier dual}\index{Cartier duality}
$N^D\defeq\shom(N,\bbG_{m,K})=\shom(N,\mu_{n,K})$ can be represented by a finite, \'etale group
scheme. Hence, it corresponds to a finite, continuous $G$-module:


\begin{prop}\label{cup_prep_DP}  % Cartier Dual, Pontrjagin dual
Let $N$ be a finite, \'etale $K$-group scheme whose order $n$ is prime to $p$. Then its Cartier dual
is \'etale and corresponds to the $G$-module $\hom(N(K_s),\bbQZ)$ with $G$-structure
\[
      (\sigma\cdot\phi)(n)\defeq\phi(\sigma(n)),
\]
for $\sigma\in G$, $\phi\in\hom(N(K_s),\bbQZ)$ and $n\in N(K_s)$. That is, Cartier duality of finite
group schemes of order prime to $p$ corresponds to Pontrjagin duality\index{Pontrjagin duality} of
$G$-modules.
\end{prop}

\begin{proof}
\enum 1. Since $N$ is \'etale, there exists a finite Galois extension $L/K$ such that $N_L\defeq
N\tensor_K L$
is constant. Since $\mu_{n,L}\iso\bbZ\mod n$ for all $n$ which are prime to $p$, we see that $N$
is 
multiplicative. Hence, its Cartier dual is \'etale, \cite{ga}, IV, \S1, 3.2.
\par
The $G$-module, corresponding to $\shom(N,\bbG_{m,K})$ is given by the abelian group
$\hom(N,K_s^\ast)$, with $G$-structure (cf.\ \cite{Br}, chapter III, section 0)
\[
(\sigma\cdot\phi)(n)\defeq\sigma\inv(\phi(\sigma(n))).
\]
As $N$ is finite and of order prime to $p$, its image in $K_s^\ast$ is contained in some
$\mu_n(K_s)$. Since $G$ acts trivially on the group of the $n$-th roots of unity of $K_s$, this
group can be embedded into the group $\bbQZ$ with trivial $G$-action.
\end{proof}




Pontrjagin duality induces the Pontrjagin  pairing
$N\times N^\ast\to\bbZ\mod n\sub\bbQ\mod\bbZ$. Combining the cup product with this pairing, we
obtain the pairing
\begin{equation}\label{cup_pairing}
\HH^0(G,N)\times\HH^1(G,N^\ast)\longto\HH^1(G,\mu_n(K_s))=\bbZ\mod n\sub\bbQZ,
\end{equation}
which again we refer to as cup product. It is an important fact that in our situation this product
is perfect:


\begin{thm}\label{cup_perf}
Let $N$ be a finite, continuous $G$-module of order prime to $p$. Then the cup product pairing of
\eqref{cup_pairing} is perfect.
\end{thm}

We need some preparations to prove this theorem:
Let us recall the functor of \emph{coinvariants} of group homology. Let $N$ be a $G$-module. Then we
define the functor of coinvariants, $N_G$ as the quotient $N\mod N'$, where $N'$ is the
subgroup of $N$, which is generated by all expressions of the shape $gn-n$, for $g\in G$ and $n\in
N$. As always, the group $N^G\defeq \HH^0(G,N)$ of invariants is defined to be the subgroup of $N$
whose elements are stable under the action of $G$.

\begin{lemma}\label{cup_prep}
Let $N$ be a finite, continuous $G$-module whose order $n$ is prime to $p$ and let $P\sub G$ be a
pro-$p$-group.
\begin{enumprop}
    \item We have $\HH^i(P,N)=0$ for $i\geq 1$.
    \item There is a canonical isomorphism $(N^G)^\ast\isoto (N^\ast)_G$.
    \item The canonical map $N^P\isoto N_P$ is an isomorphism.
\end{enumprop}
\end{lemma}


\begin{proof}
Statement \enum 1:  Let $P'\sub P$ be an open subgroup of index $p^n$. The composition of
restriction and corestriction $\HH^i(P/P',N)\to\HH^i(e,N)\to\HH^i(P/P',N)$ is multiplication with
$p^n$. Since the order of $N$ is prime to $p$, this map is bijective. Moreover it is trivial,
because the map factorises over the trivial group $\HH^i(e,N)$. This implies \enum 1.
\par
Statement \enum 2 can be seen as follows: The Pontrjagin dual $\hom(-,\bbQZ)$ defines an
auto-duality of the category of finite groups. In particular, it takes projective limits to
inductive ones and kernels to cokernels. Using the equalities
\begin{align*}
N^G = & \projlim_{\sigma\in G}\ker (N\Longto{\sigma-1} N), \\
N_G = & \indlim_{\sigma\in G} \coker(N\Longto{\sigma-1} N),
\end{align*}
assertion \enum 2 follows.
\par
Finally, let us show \enum 3. We define $N'$ by the exact sequence
\[
0\longto N'\longto N\longto N_P\longto 0.
\]
It induces the sequence
\[
\HH^0(P,N)\longto\HH^0(P,N_P)\longto\HH^1(P,N').
\]
As the order of $N'$ is prime to $p$, the right cohomology group vanishes. Therefore the
homomorphism $f\colon N^P\to N_P$ is surjective. The same argument shows that there is a surjection
$(N^\ast)^P\onto (N^\ast)_P$. With \enum 2 we see that this homomorphism can be written as
a surjection $(N_P)^\ast\onto (N^P)^\ast$. Hence, $f$ must be injective, too.
\end{proof}



Finally, we need some facts of group cohomology, \cite{cg}, chap. I, p.\ 3:

\begin{lemma}\label{hatZ}
We have the equalities $\HH^0(\hat\bbZ,N)=N^{\hat\bbZ}$ and $\HH^1(\hat\bbZ,N)=N_{\hat\bbZ}$. \qed
\end{lemma}

Before we prove the theorem, let us recall the exact sequence of corollary \ref{galK_seq} which
describes the Galois group $G=\gal(K_s/K)$:
\[
0\longto P\longto G\longto H \longto 0
\]
with $H\defeq \prod_{\ell\neq p}\hat\bbZ_\ell$ and a pro-$p$-group $P$.

\begin{proofof}{Theorem \ref{cup_perf}}
From the Hochschild-Serre spectral sequence
\[
\HH^r(H,\HH^s(P,N))\ssto\HH^{r+s}(G,N)
\]
and lemma \ref{cup_prep}, \enum 1 we obtain isomorphisms
\[
\HH^i(H,N^P)\isoto\HH^i(G,N)\quad\text{for all $i$.}
\]
\par
As $\hat\bbZ\iso H\oplus\hat\bbZ_p$ we can equip $N^P$ with a $\hat\bbZ$-action: Elements of $H$
act as before, elements of $\hat\bbZ_p$ act trivially. By the spectral sequence
\[
\HH^r(H,\HH^s(\hat\bbZ_p,N^P))\ssto\HH^{r+s}(\hat\bbZ,N^P)
\]
together with lemma \ref{cup_prep}, \enum 1,  we obtain isomorphisms
\[
\HH^i(\hat\bbZ,N^P)\isoto\HH^i(H,N^P)\isoto\HH^i(G,N)\quad \text{for all $i\in\bbN$}.
\]
Now, the cup product of the theorem can be written as
\begin{equation}\label{cup_prod1}
\HH^0(\hat\bbZ,N^P)  \times  \HH^1(\hat\bbZ,(N^\ast)^P) \longto \bbQZ.
\end{equation}
Again, by lemma \ref{cup_prep}, \enum 2 and \enum 3, there are isomorphisms
\[
(N^P)^\ast\isoto (N^\ast)_P\isoto (N^\ast)^P.
\]
It induces the following isomorphism on cohomology:
\[
\HH^1(\hat\bbZ,(N^\ast)^P)\isoto\HH^1(\hat\bbZ,(N^P)^\ast).
\]
Let us write $M\defeq N^P$. Using lemma \ref{hatZ}, we can write the cup product of
\eqref{cup_prod1} as
\[
M^{\hat\bbZ}\times (M^{\hat\bbZ})^\ast\longto\bbQZ.
\]
This is the perfect Pontrjagin pairing.
\end{proofof}




\label{cup_all_sits}The perfect cup product is of great help in the study the cohomology of $K$. As
we have seen, it
depends severely on the structure of the Galois group $\gal(K_s/K)$. We will see later that cup
products do not only exist for Galois- and \'etale cohomology but also for the smooth and the flat
topology. We will deduce a comparison theorem that all these cup products coincide, once the
cohomology groups coincide. Hence, we can read  theorem \ref{cup_perf} relatively to the \'etale or
the flat topology and obtain a perfect pairing 
\[ 
\HH^0(K,N)\times\HH^1(K,N^D)\longto\bbQZ 
\] 
on
either site. This pairing will be the central cohomological tool to show that Grothen\-dieck's
pairing for abelian varieties is perfect on its prime-to-$p$-part. Later, we will construct an
alternate pairing that can be seen as a replacement for the cup product for certain $p$-groups.

